RP-Rewriter: An Optimized Rewriter for Large Terms in ACL2

RP-Rewriter (Retain-Property) is a verified clause processor that can use some of the existing ACL2 rewrite rules to prove conjectures through term rewriting. Optimized for conjectures that can expand into large terms, the rewriter tries to mimic some of the ACL2 rewriting heuristics but also adds some extra features. It can attach side-conditions to terms that help the rewriter retain properties about them and prevent possibly some very expensive backchaining. The rewriter supports user-defined complex meta rules that can return a special structure to prevent redundant rewriting. Additionally, it can store fast alists even when values are not quoted. RP-Rewriter is utilized for two applications, multiplier design proofs and SVEX simplification, which involve very large terms.

==> eptcsdata.tex <==
\providecommand{\firstpage}{61}
\providecommand{\publicationstatus}{G. Passmore, R. Gamboa (Eds.): ACL2 Workshop 2020\\
EPTCS 327, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.327.5}{10.4204/EPTCS.327.5}}

